Multiscale Linear-Quadratic Stochastic Optimal Control With Multiplicative Noise

We investigate the asymptotic properties of a finite-time horizon linear-quadratic optimal control problem driven by a multiscale stochastic process with multiplicative Brownian noise. We approach the problem by considering the associated differential Riccati equation and reformulating it as a classical and deterministic singular perturbation problem. Asymptotic properties of this deterministic problem can be gathered from the well-known Tikhonov Theorem. Consequently, we are able to propose two approximation methods to the value function of the stochastic optimal control problem. The first is by constructing an approximately optimal control process whilst the second is by finding the direct limit to the value function. Both approximation methods rely on the existence of a solution to a coupled differential-algebraic Riccati equation with certain stability properties - this is the main difficulty of the paper.

==> packages.tex <==
%\usepackage{T1enc}

%\usepackage{multicol}    % used for the two-column index
\usepackage{upgreek}
%\usepackage{algorithmic}
%\usepackage[square]{natbib}
%\bibpunct[; ]{(}{)}{,}{a}{}{;} 
%\usepackage{a4}
\usepackage{wrapfig}
\usepackage{boxedminipage}
%\usepackage{boites} 
\usepackage{pifont}
%\usepackage{tweaklist}
%\usepackage{algorithmicx}
%\usepackage{algpseudocode}
%\usepackage{algmatlab}
\usepackage{euscript}
\usepackage{dcolumn}
%\usepackage{fancyheadings}
\usepackage{float}
\usepackage{fancybox}
\usepackage{rotating}
\usepackage{multirow}
\usepackage{latexsym}
\usepackage{amssymb}
\usepackage{txfonts}
\usepackage{amsmath}
%\usepackage{amsthm}  % gives different style
\usepackage{epsfig}
\usepackage{color}
\usepackage{verbatim}
\usepackage{subfigure}
\usepackage{mathrsfs}
\usepackage{url}
\usepackage{lscape}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Post Script Font File(s)

% For TimesRoman Math (You must have MathTimes and MathTimes Plus 
%                        font sets, order fonts from  www.yandy.com)
% \usepackage[mtbold,noTS1]{m-times}

% For PostScript text
%\usepackage{w-bookps}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Graphicx.sty for Including PostScript .eps files

%% If you don't have graphicx.sty available, unzip the graphics.zip
%% file included in this package.

% Choose one of these options, based on the system that you are using.
% If none look like your system, use dvips
% [dvips], [xdvi], [dvipdf], [dvipsone], [dviwindo], [emtex], [dviwin],
% [pctexps],  [pctexwin],  [pctexhp],  [pctex32], [truetex], [tcidvi],
% [oztex], [textures]

\usepackage{graphicx}

%\usepackage{hyperref} %Automatic hyperlinks in pdf.

